Time Dependence in Kalman Filter Tuning

In this paper, we propose an approach to address the problems with ambiguity in tuning the process and observation noises for a discrete-time linear Kalman filter. Conventional approaches to tuning (e.g. using normalized estimation error squared and covariance minimization) compute empirical measures of filter performance and the parameter are selected manually or selected using some kind of optimization algorithm to maximize these measures of performance. However, there are two challenges with this approach. First, in theory, many of these measures do not guarantee a unique solution due to observability issues. Second, in practice, empirically computed statistical quantities can be very noisy due to a finite number of samples. We propose a method to overcome these limitations. Our method has two main parts to it. The first is to ensure that the tuning problem has a single unique solution. We achieve this by simultaneously tuning the filter over multiple different prediction intervals. Although this yields a unique solution, practical issues (such as sampling noise) mean that it cannot be directly applied. Therefore, we use Bayesian Optimization. This technique handles noisy data and the local minima that it introduces.

==> BayesOpt_Background.tex <==
%%
%%\nisarcomm{text in this part is from recently published JAIS paper: need to modify text, and trim for space and, modify for notation...}

Consider the minimization of an objective function $y:\bovarspace \rightarrow \mathbb{R}$, where $\bovarspace \in \mathbb{R}^d$ is the search or solution space, and $\bovar^* \in \bovarspace$ is the minimizer, such that $y(\bovarspace^*) \leq y(\bovarspace), \  \forall \bovar \in \bovarspace$.
Furthermore, we assume that each elements of $i$ of $\bovar$ lies in the interval $\bovarspace (i) \in [\bovar(i)_l, \bovar(i)_u]$. the goal of Bayesian optimization is to find the minimizer of the noisy objective function $\fy$
while at the same time learning about the mapping from $\bovar$ to $\fy$ via Bayesian inference.% for lower bound $\bovar(i)_l$ and upper bound $\bovar(i)_u$ for element . 
%When the mapping from $\bovar$ to $\fy$ is not known explicitly, optimization typically requires the evaluation of a `black box' function. 
%In the present application, $\fy$ is the objective function for filter auto-tuning; this will be defined later in Section \ref{sec:stochcosts} via stochastic functions which provide simulation-based or observation residual-based measures of Kalman filter performance. %so called JNIS in equation \ref{JNIS_def}, which basically uses the sensor data in Kalman Filter to indicate the performance of Kalman Filter so the ground-truth is not needed. -->nra: too early to mention this part; will not make sense until later.

%The intuition behind BO arises from the following. First suppose that the entire solution space was densely sampled. Carrying out this process, the map $y:\bovarspace \rightarrow \mathbb{R}$ is entirely known and the minimizer can be read off directly. However, this dense sampling scheme is not possible in practice. Rather, the search algorithm samples a subset of the parameter space. Since the sampling is incomplete, the shape of the cost surface is not known but, rather, must be estimated from sparse and incomplete data.
%Therefore, the goal of Bayesian optimization is to find the minimizer of the noisy objective function $\fy$
%while at the same time learning about the mapping from $\bovar$ to $\fy$ via Bayesian inference. Bayesian optimization uses ``black box'' point evaluations of $y$ to efficiently find $\bovar^*$. This is accomplished by maintaining beliefs about how $\fy$ behaves over all $\bovar$ in the form of a surrogate model $\fs$, which statistically approximates $\fy$ and is easier to evaluate (e.g. since evaluations of $\fy$ might require expensive high-fidelity simulation). During optimization, $\fs$ is used to determine where the next design point sample evaluation of $\fy$ should occur, in order to update beliefs over $\fy$ and thus simultaneously improve $\fs$, while finding the (expected) minimum of $\fy$ as quickly as possible. The key idea is that, as more observations $E$ are sampled at different $\bovar$ locations, the $\bovar$ samples themselves eventually converge to the expected minimizer $\bovar^*$ of $\fy$. Since $\fs$ contains statistical information about the level of uncertainty in $\fy$ (i.e. related to the posterior belief $p(y|E)$), Bayesian optimization effectively leverages probabilistic ``explore-exploit'' behavior to learn a probabilistic model of $\fy$ while also minimizing it.

\indent There are the two main components of the Bayesian optimization process: (1) The surrogate model $\fs$, which encodes statistical beliefs about $\fy$. (2) The acquisition function is used to intelligently guide the search for $\bovar^*$ via $\fs$.
\subsubsection{Surrogate Model}
\indent The surrogate model is the model used to approximate the objective function. We use the Student-t process as we discussed in this section's first part %In the BO literature, nonparametric regression models based on stochastic processes are widely used~\cite{rasmussen2003gaussian} because they naturally model probability distributions over uncertain functions and can be evaluated at arbitrary query points given some finite set of sample observation points. %, nonparametric regression models lead to natural prior and posterior distributions for $\fy$ that can subsequently be used to derive surrogate functions $\fs$. 
%Although Gaussian process (GP) is frequently used \cite{garnett2010bayesian}, \cite{rana2017high}, \cite{djolonga2013high}, in this work we use Student-t processes (TP) instead, following the recommendation of Shah, et al.\ \cite{shah2014student}. %that it could be  useful to replace GP with TP in almost any application. %\sjj{what recommnendation is that?}

%\sjj{Shouldn't we change this to Student-t instead?} \zzc{change student's-t to student-t}


\indent A Student-t process is a stochastic process such that every finite collection of samples from the process has a multivariate Student-t joint distribution. The mean function $\Phi(\mathbf{q})$, the kernel function $k(\mathbf{q})$ and the parameter $v$ are the main characteristics of TP. It can be written as 
\begin{equation}
    y(\mathbf{q}) \sim \mathcal{TP}(v, \Phi(\mathbf{q}), k(\mathbf{q},\mathbf{q}')).
\end{equation}
The real-valued parameter $v>2$ controls how ``heavy-tailed'' the process is. The heavier the tail (i.e. the smaller the $v$), the more likely it is that the TP will produce a value that is far from the mean value. The TP tends to a GP as $v \rightarrow \infty$. %The reason we choose the T Process is that 
The TP is attractive because it provides some extra benefits over GP, without incurring more computational cost. For example, the predictive covariance for the TP explicitly depends on observed $y$ data values; this is a useful property which the Gaussian process lacks. Furthermore,  distributions over the cost function $y$ may in general be heavy-tailed, so it is better to use TP to ``safely'' model their behaviors \cite{shah2013bayesian}. Similarly, every finite collection of TP samples $\mathbf{q}_{1:n} = (\mathbf{q}_1, \mathbf{q}_2, \cdots, \mathbf{q}_n)$ has a multivariate Student-t distribution, which can be written as \\
\begin{align} \label{mvt}
\begin{split}
    & y(\mathbf{q}_{1:n}) = \frac{\Gamma(\frac{v+n}{2}) }{\Gamma(v/2)((v-2)\pi)^{n/2}|K|^{1/2}} \\
    & \times (1 + \frac{1}{v-2}(\mathbf{q}_{1:n} - \Phi(\mathbf{q}_{1:n})^TK^{-1}(\mathbf{q}_{1:n} - \Phi(\mathbf{q}_{1:n}))^{-\frac{v+n}{2}}
\end{split}
\end{align}
\noindent where $\Gamma(n)$ is the gamma function for $n\in \mathbb{R}$, %$\Gamma(n) = (n-1)!, \ n \in \mathbb{R}$ 
and $v>2$. $K$ is the covariance matrix consisting of kernel function $k$ \cite{Rasmussen2006}, \cite{minasny2005matern}, \cite{genton2001classes} evaluations,
\begin{equation} \label{cov_matrix}
    K = 
    \begin{bmatrix}
    k(\mathbf{q}_1, \mathbf{q}_1) & k(\mathbf{q}_1, \mathbf{q}_2) & \cdots & k(\mathbf{q}_1, \mathbf{q}_n) \\
    k(\mathbf{q}_2, \mathbf{q}_1) & k(\mathbf{q}_2, \mathbf{q}_2) & \cdots & k(\mathbf{q}_2, \mathbf{q}_n) \\
    \vdots & \vdots & \vdots & \vdots \\
    k(\mathbf{q}_n, \mathbf{q}_1) & k(\mathbf{q}_n, \mathbf{q}_2) & \cdots & k(\mathbf{q}_n, \mathbf{q}_n)
    \end{bmatrix}.
\end{equation}
Equation (\ref{mvt}) is written as the following for simplicity,
\begin{equation}
    y(\mathbf{q}_{1:n}) \sim MVT_n(v, \Phi(\mathbf{q}_{1:n}), K).
    \label{eq:mvt}
\end{equation}
For Bayesian optimization, newly sampled $\bovar$ and $y$ values are added to the vector $\mathbf{q}_{1:n}$ and $y(\mathbf{q}_{1:n})$ to construct a surrogate model of the underlying objective function according to Eq.\ (\ref{eq:mvt}). In most implementations of Bayesian optimization, as the new sample values are added, the hyperparameters for the kernel function $k$ are also re-estimated from the available data and updated accordingly. The updated surrogate model is then used to compute the acquisition function, which is used to select the next sample $\bovar$ for evaluation of $y$. 
%%\indent The current $MVT$ will be the current `Surrogate Model' as we have mentioned before and they are used to to decide the next point for Bayesian Optimization to sample \nra{need to clarify meaning of this sentence...}. Now we'll discuss how to decide the next point.
%%\nra{tweaked description to also mention hyperparams for kernel, which also need to be updated}
\begin{figure*}[htbp!] %figure's label should be after caption
    \centering
	\includegraphics[width=180mm]{figs/bayesopt-ekf.png}
    \caption{System Flowchart: Bayesian optimization will fit a surrogate model based on some sampled input parameters and associated costs according to the ``black box'' objective function, and then starts iterating until a minimum cost is found. %\nra{need to change/remove $J_{NEES}$ if it's not being used? use variables for process and measurement noises in second block on top (yellow) and on bottom (peach)?  also from text comment: move this to sec 3.}\zzc{delete JNEES but the software I use to generate the picture don't support latex... Next time I'll try to use latex or markdown to generate to the flow chart}
    }  \label{PG1} %progress 1
\label{xfigDiagram}
\end{figure*}

\subsubsection{Acquisition Function}
The expected improvement function is one of many well-known acquisition functions; other possible and popular choices for the acquisition function include the \emph{Lower Confidence Bound (LCB)}. We use expected improvement function in of our implementations and we'll discuss how this acquisition function is generated next. Suppose that $n$ points $\mathbf{q}_{1:n}$ and $y(\mathbf{q}_{1:n})$ have been sampled and have been incorporated into the surrogate model. The current minimizer is $\mathbf{q}^*_{1:n}=\min_{m \leq n}y(\mathbf{q}_m)$. This will be one of these points, since observations of $y$ are not available for other points in $\bovarspace$. The algorithm needs to choose the next point $\mathbf{q}_{n+1}$ to be sampled. We seek a new location which will yield a new, lower, minimum. In other words, $y(\mathbf{q}_{n+1})<y(\mathbf{q}^*_{1:n})$. 
%the current minimizer's observation. 
One way to evaluate the new sample point is to evaluate its 
\emph{improvement} with respect to $\mathbf{q}^*_{1:n}$
\begin{equation}
    g(\mathbf{q}_{n+1}, \mathbf{q}^*_{1:n}) = \max(0, y_n(\mathbf{q}^*_{1:n}) - y(\mathbf{q}_{n+1})).
\end{equation}
This only assigns a non-zero value if  $\mathbf{q}_{n+1}<\mathbf{q}^*_{1:n}$. Therefore, the idea is to chose $\mathbf{q}_{n+1}$ which maximizes the improvement. Since we only have access to the surrogate function, the improvement is stochastic. Therefore, we choose the next sample point based on the \emph{expected improvement} 
\begin{equation} \label{expected_improvement}
    E_n[g(\mathbf{q}_{n+1}, \mathbf{q}^*_{1:n}) \ | \ \mathbf{q}_{1:n}, \mathbf{y}(\mathbf{q}_{1:n}) ]
\end{equation}
\noindent $E_n[\cdot]$ is the expectation based on current posterior distribution, given by the current $MVT$ surrogate model. We need maximize Eq.\ \ref{expected_improvement} to find the next point to sample.
\begin{equation}
    \mathbf{q}_{n+1} = \argmax\limits_{\mathbf{q}_{n+1}} E_n[g(\mathbf{q}_{n+1}, \mathbf{q}^*_{1:n}) \ | \ \mathbf{q}_{1:n}, \mathbf{y}(\mathbf{q}_{1:n}) ]
\end{equation}
The closed form solution of the $\mathrm{EI}$ acquisition function using the TP surrogate is \cite{shah2013bayesian, tracey2018upgrading},
\begin{align} \label{EI_function}
    \mathrm{EI}_n(\mathbf{q}) = \left(y_n(\mathbf{q}^*_{1:n}) - u\right)\Psi(z) + \frac{v}{v-1}\left(1 + \frac{z^2}{v}\right)\sigma \psi(z)
\end{align}
\noindent where $u$ and $\sigma$ are the mean and variance of the conditional Student's-t distribution of $\mathbf{q}_{n+1}$, which is presented below in \eqref{con_MVT}.  $\Psi(\cdot)$ and $\psi(\cdot)$ are the CDF and PDF of the standard Student-t distribution $MVT_1(v, 0, 1)$. The conditional $MVT$ distribution is similar to the conditional multivariate Gaussian distribution: if we have $\mathbf{q}_{1:n+1}$ and $y(\mathbf{q})_{1:n+1}$ described by a multivariate $MVT$ pdf, then 
\begin{align} \label{MVT_nplus1}
    \begin{split}
    \begin{bmatrix}
        y(\mathbf{q}_{1:n}) \\
        y(\mathbf{q}_{n+1})
    \end{bmatrix}
    & \sim 
    MVT_{n+1} \left(v+1,
    \begin{bmatrix}
        \Phi(\mathbf{q}_{1:n}) \\
        \Phi(\mathbf{q}_{n+1}) \\
    \end{bmatrix} \right|
    , \\
    & \left|\begin{bmatrix}
        K(\mathbf{q}_{1:n}, \mathbf{q}_{1:n}) & K(\mathbf{q}_{1:n}, \mathbf{q}_{n+1}) \\
        K(\mathbf{q}_{n+1}, \mathbf{q}_{1:n}) & K(\mathbf{q}_{n+1}, \mathbf{q}_{n+1}) \\
    \end{bmatrix} \right)
    \end{split}
\end{align}
where $K(\mathbf{q}_{1:n}, \mathbf{q}_{1:n})$ is the same as eq. (\ref{cov_matrix}), $K(\mathbf{q}_{1:n}, \mathbf{q}_{n+1}) = [k(\mathbf{q}_1 , \mathbf{q}_{n+1}), \cdots, k(\mathbf{q}_n , \mathbf{q}_{n+1})]^T$, and $K(\mathbf{q}_{n+1}, \mathbf{q}_{n+1}) = k(\mathbf{q}_{n+1} , \mathbf{q}_{n+1})$. %For simplification, we'll rewrite equation 
\eqref{MVT_nplus1} can be written more simply as
\begin{equation} \label{sim_MVT_nplus1}
    \begin{split}
    \begin{bmatrix}
        y_1 \\
        y_2
    \end{bmatrix}
    \sim 
    MVT_{n+1}\left(v+1,
    \begin{bmatrix}
        \Phi_1 \\
        \Phi_2 \\
    \end{bmatrix}
    , 
    \begin{bmatrix}
        K_{11} & K_{12} \\
        K_{21} & K_{22} \\
    \end{bmatrix} \right)
    \end{split}
\end{equation}
The conditional Student-t distribution of $y(\mathbf{q}_{n+1})$ is then given by \cite{ding2016conditional}
\begin{equation} \label{con_MVT}
    \begin{split}
        & y(\mathbf{q}_{n+1}|\mathbf{q}_{1:n}, y(\mathbf{q}_{1:n})) \sim MVT_1(v+n, u, \sigma) \\
        & u = \Phi_2 + K_{21}K_{11}^{-1}(y_1 - \Phi_1) \\
        & \sigma = \frac{v+d}{v+n} K_{22}-K_{21}K_{11}^{-1}K_{12} \\
        & d = (y_1 -  \Phi_1)^T K_{11}^{-1}(y_1 - \Phi_1)
    \end{split}
\end{equation}
The prior mean function for the surrogate model in Bayesian optimization can be set as a constant %(e.g. 0) 
without changing the final result \cite{brochu2010tutorial}, %which means we can 
so let $\Phi_1 = \mathbf{0}, \Phi_2 = 0$. Substituting Eq.\ (\ref{con_MVT}) into Eq.\ (\ref{EI_function}), the only unknown variable will be $\mathbf{q}_{n+1}$. To find the $\mathbf{q}_{n+1}$ that maximizes Eq.\ \eqref{EI_function} for the largest improvement, another inner optimization problem must be solved within Bayesian optimization. Luckily, Eq.\ \eqref{EI_function} is known, there are several ways to maximize the $\mathrm{EI}$ function, such as \emph{DIRECT} \cite{finkel2003direct}, which is a derivative free and deterministic nonlinear global optimization algorithm that is widely used for Bayesian optimization via nonparametric surrogate model regression. Once the next point to sample is selected by the inner loop optimization, the Bayesian optimization loop can continue until the termination criterion (maximum iteration or minimum observation change between two iterations) is met.

The resulting algorithm for Bayesian optimization is referred to here as \BO{} (Student-t processes Bayesian optimization).



==> basic_example.tex <==
\section{Basic Example}
\label{eqn:basic_example}

For practical use, all of our applications consider continuous to discrete transformation with a sample time $\Delta t$. The first example is a 1D tracking system. Consider a robot that moves along a 1D track and receives position measurements
every time step. The system state, 
$\x{} = [x,
\dot{x}]^T$, evolved overtime according tothe  are governed by the linear time invariant model
\begin{equation}
\label{eq:con_sys_model}
\begin{aligned}
\dot{\mathbf{x}}_t &= \mathbf{A} \x{t} + \mathbf{G} \uVec{t} + \mathbf{\Gamma} \vVec{t} \\
\z{t} &= \HM{} \x{t} + \wVec{t}
\end{aligned}
\end{equation}
\noindent where 
\begin{align*}
\mathbf{A} =
\begin{bmatrix}
0 & 1 \\
0 & 0 
\end{bmatrix}, \ \ 
\mathbf{G} =
\begin{bmatrix}
0 \\
1  
\end{bmatrix}, \ 
\HM{} =
\begin{bmatrix}
1 & 0  
\end{bmatrix}, \ 
\mathbf{\Gamma} = 
\begin{bmatrix}
0 \\ 
1  
\end{bmatrix}. \ 
\end{align*}
The inputs to the system are: a control acceleration $\uVec{t}$, additive white Gaussian noise acceleration process $\vVec{t}$ with intensity $\V$, and additive white Gaussian position measurement noise process $\wVec{t}$ with continuous time intensity $\W$. In the measurement part, we assume we only measure the position and in the process part, we assume only the speed has additive noise so $\V$ and $\W$ are both scalars, $\V = v$, $\W = \omega$. The control input is set as $\uVec{t}=2\cos(0.75t)$, it causes the robot to move with a low frequency oscillation. Applying a zero-order hold discretization to this system, we obtain discrete time position and velocity state $\x{\kCur} = [x, \dot{x}]^T$ and the linear time-invariant parameters for eqs. (\ref{eq:dynModel})-(\ref{eq:measModel}), the discrete time system can be computed by the following equation
\begin{equation}
\begin{aligned}
&\F{} = 
e^{\mathbf{A}\Delta t}, \ \
\mathbf{B} = 
\int_{0}^{\Delta t} e^{\mathbf{A} m} \mathrm{d} m, \ \
\R{} =  \frac{\W}{\Delta t}\\
&\Q{} =  \int_{0}^{\Delta t} e^{\mathbf{A}m} \mathbf{\Gamma} \V \mathbf{\Gamma}^T e^{\mathbf{A}^Tm} \mathrm{d} m 
\label{eq:VanLoans}
\end{aligned}
\end{equation}
The discrete time plant is computed using Van Loan's method \cite{BrownHwang2012}. Thus, we can get the discrete system
\begin{equation}
\begin{aligned}
&\F{} = 
\begin{bmatrix}
1 & \Delta t \\
0 & 1
\end{bmatrix}, \ \
\mathbf{B} = 
\begin{bmatrix}
0.5 \Delta t^2 \\
\Delta t
\end{bmatrix}, \ \ 
\HM{} = 
\begin{bmatrix}
1 & 0
\end{bmatrix}\\
&\Q{} = v\begin{bmatrix}
 \frac{1}{3} \Delta t^3 & \frac{v}{1} \Delta t^2 \\
 \frac{1}{2} \Delta t^2 & \Delta t
\end{bmatrix}, \ \ \R{} = \frac{\omega}{\Delta t}
\end{aligned}
\label{eq:covariance_definitions}
\end{equation}
Both the discrete process noise covariance $\mathbf{Q}$ and the observation noise covariance $\mathbf{R}$ are functions of $\Delta{t}$

%\sjj{Can we provide an initial example which illustrates why cnis is required?}\zzc{The result of the 1D tracking system cannot show the Cnis is better... Use Cnis or original Jnis is almost the same for the 1D system. I found the problem that the mean and variance doesn't match when I test the 2D tracking system. If I need to raise an example, I need to introduce the experiment system first...  Finally I answer this question in the last section of the experiment...}

%We can see if we need to calculate the NIS and finally the $\Cnis$, the value of them is highly non-linear with respect to $\Delta t$ besides the continuous noise intensity $\mathbf{W}$ and $\mathbf{V}$. To the best of our knowledge, the relationship between $\Delta t$ and the NIS related cost has never been investigated. 


==> bayesopt.tex <==
\section{Bayesian Optimization based Tuning}
\label{sct:bayesopt}

%bayesopt.tex

%Bayesian optimization arises from following idea. If the value of the cost function were known everywhere, the minimum could trivially be chosen. However, to do this we would have to exhaustively compute the costs everywhere. Instead, we only get a subset of observations. As a result, there is uncertainty 

Many approaches for solving nonlinear optimization problems use gradient descent. However, the risk with these approaches is that they can fall into local minima. This issue is exacerbated for filter tuning problems defined by noisy nonlinear dynamical systems. %With a finite number of samples, 
Stochastic variations and nonlinear model characteristics can introduce many local minima into objective functions for tuning that can trap gradient descent methods. One principled way to handle such cases is to use \emph{Bayesian optimization\/} (BO) \cite{pelikan1999boa}, which poses optimization as a probabilistic search problem. In the BO literature, nonparametric regression models based on stochastic processes are widely used~\cite{rasmussen2003gaussian} because they naturally model probability distributions over uncertain functions and can be evaluated at arbitrary query points given some finite set of sample observation points.
Although Gaussian process (GP) is frequently used \cite{garnett2010bayesian}, \cite{rana2017high}, \cite{djolonga2013high}, in this work we use Student-t processes (TP) instead, following the recommendation of Shah, et al.\ \cite{shah2014student} that the TPBO increases modelling flexibility at no extra cost and still hold the GPBO benefits.\\
\indent Bayesian optimization is first described for dealing with generic ``black box'' stochastic objective functions. Its novel application is then described for simulation-based Kalman filter auto-tuning then. %We won't go to the detail of BO because it is explained in detail in out previous work \cite{chen2018weak}. We'll simply point out the key point of the BO and address the difference between the BO using in this work and our previous work.
% star* makes it can cross two columns


\subsection{Bayesisan Optimization Theory}
\label{subsct:BA_theory}
\input{BayesOpt_Background.tex}


\subsection{Tuning Algorithm Summary} \label{subsct: summary}
Algorithm \ref{alg:BayesOpt} summarizes the \BO{} procedure for Kalman filter tuning. % The termination criteria could be based on iteration thresholds, tolerances on changes to the optimum $\bovar$ and/or $\fy$ between iterations, or other methods. 
 An attractive feature of \BO{} is that it naturally provides uncertainty quantification on the shape of the objective function at both sampled and unsampled locations. This allows \BO{} to cope with multiple local minima in the parameter space $\bovarspace$.
%However, in practice, the \BO's performance depends on the selection and parameterization of the surrogate model kernel, as well as the number and placement of initial training observations (i.e. seed points) to bootstrap the search process. 

%\nra{need a paragraph in here to back up the contribution claims about NIS cost function made in beginning in the abstract and introduction -- both NEES and NIS are described here as in the FUSION conference paper, but should there be a bit more discussion/remarks here about why NIS is `preferable' to NEES, since NIS doesn't require ground-truth state data? Or should the intro/abstract be re-written to claim both NEES and NIS are novel/useful contributions?} \zzc{I think `no need of groundtruth` should be a strong enough reason? In part \ref{previous_work} I have both said the strength of NIS and our previous work using NEES. I guess that should be enough?}

{\centering
\begin{minipage}{.92\linewidth}

 \begin{algorithm}[H]
            % Bayesian optimization procedure
            \caption{\BO{} for Kalman filter tuning}
            \label{alg:BayesOpt}
            \begin{algorithmic}[1] % The number tells where the line numbering should start
                    \State Initialize TP with seed data $\left\{\bovar_s, \fy_s\right\}_{s=1}^{N_{seed}}$ and hyperparameters $\Theta$
                    \While {termination criteria not met}
                        \State $\bovar_j = \argmax_{\bovarspace} \fa$ %\Comment equation \ref{eq:EI1} when applying the EI criterion
                        \State Evaluate $y(\bovar_j)$, e.g., $\Cnis(\bovar)$. on two different $\Delta t$. Choose the larger one as $y(\bovar_j)$ 
                        \State Add $y(\bovar_j)$ to $\fv(Q)$, $\bovar_j$ to $Q$, and update $\Theta$ \label{ln:testing}%\Comment see Sec. \ref{sec:MLE_MAP_CV} 
                    \EndWhile \\
                    \Return $\bovar^* = \arg \min_{\bovar_j \in Q} \fv(\bovar_j)$
            \end{algorithmic}
        \end{algorithm}
\end{minipage}
\par
}
Based on samples over the system input and
corresponding outputs from the objective function,
Bayesian optimization fits a surrogate model of the ``true''
objective function. The optimization method then repeats this process to find a minimum of the current surrogate model, update this surrogate model, and find the minimum of the new surrogate model until pre-set termination conditions are met. Note that based on the conclusion from Section \ref{sct:observability}, we know only around the groundtruth value the $\Cnis$ can be consistent and small whatever the $\Delta t$ is. Based on this, for the same noise intensity set, we simply evaluate the $\Cnis$ twice on different $\Delta t$, choose the larger $\Cnis$ and feed it into BO. Thus, we force the BO to choose small $\Cnis$ on both $\Delta t$. Theoretically, according to Figure \ref{fig:tracking1d_gt}, \ref{fig:tracking2d_gt}, for every set noise parameter, if we can run KF on numerous different $\Delta t$, accumulate the $\Cnis$ and calculate its mean and variance for BO, we can ensure the optimized parameter has small $\Cnis$ on all $\Delta t$. However, this approach is time-consuming and not realistic because the physical system may not be able to have too many sample time choices. In our experiment, two different $\Delta t$ such as $0.5s$ and $0.1s$ are sufficient for a promising optimized result. Although in the experiment part we choose $0.5s$ and $0.1s$, any combination that has about $0.5s$ difference can yield satisfying result. The sample time shouldn't be too large such as $10s$. According to the \cite{wahlstrom2014discretizing}, when the sample time is too large, the Van Loan's method lost accuracy. Figure \ref{PG1} shows the key steps for the KF-Bayesian optimization
tuning procedure. %are shown in .\\
\indent After the iteration starts, we can see in the flow chart that we maximize
the acquisition function. The new point that can maximize the acquisition function will be chosen as the next set of
process noise to run the KF system. After running the KF system with the new
set of process noise we can get a new cost, which will be used to update the
surrogate model.


==> tuning.tex <==
\section{Tuning}
\label{sct:tuning}

T
